Ariadne: Analysis for Machine Learning Program

Machine learning has transformed domains like vision and translation, and is now increasingly used in science, where the correctness of such code is vital. Python is popular for machine learning, in part because of its wealth of machine learning libraries, and is felt to make development faster; however, this dynamic language has less support for error detection at code creation time than tools like Eclipse. This is especially problematic for machine learning: given its statistical nature, code with subtle errors may run and produce results that look plausible but are meaningless. This can vitiate scientific results. We report on Ariadne: applying a static framework, WALA, to machine learning code that uses TensorFlow. We have created static analysis for Python, a type system for tracking tensors---Tensorflow's core data structures---and a data flow analysis to track their usage. We report on how it was built and present some early results.

==> implementation.tex <==
\section{Implementation}

 Our implementation is in its early stages, but much of the foundation for analysis of Tensorflow code exists.   The code is all on GitHub at \url{https://github.com/wala/ML}.
\begin{description}
\item[Python 2.7 front end] We use Python's support for generating AST to create the language-specific ASTs that we need.  We use the Jython 2.7.1 implementation of Python to ease integration with WALA, which is in Java.  Given that AST, we generate WALA IR as discussed in Section~\ref{front-end}.
\item[Call graphs and pointer analysis] Given the WALA IR we generate from Python, we use the standard WALA pointer analysis and call graph construction almost unchanged, adding just small extensions to handle the Python-specific IR extensions presented in Section~\ref{python-ir}.
\item[Tensorflow model] In order to analyze code using Tensorflow rather than plain Python code, we created a model of the Tensorflow semantics as shown in Section~\ref{tf-model}.  It is integrated into call graph construction using standard WALA mechanisms, and provides IR that models the framework.
\item[Tensor types] We have a basic implementation of the types from Section~\ref{sec:types}; it constructs the appropriate tensor types for {\tt reshape} calls that appear in the code, and it does type propagation based on data flow from pointer analysis.
\end{description}

